Learning Precise, Contact-Rich Manipulation through Uncalibrated Tactile Skins

While visuomotor policy learning has advanced robotic manipulation, precisely executing contact-rich tasks remains challenging due to the limitations of vision in reasoning about physical interactions. To address this, recent work has sought to integrate tactile sensing into policy learning. However, many existing approaches rely on optical tactile sensors that are either restricted to recognition tasks or require complex dimensionality reduction steps for policy learning. In this work, we explore learning policies with magnetic skin sensors, which are inherently low-dimensional, highly sensitive, and inexpensive to integrate with robotic platforms. To leverage these sensors effectively, we present the Visuo-Skin (ViSk) framework, a simple approach that uses a transformer-based policy and treats skin sensor data as additional tokens alongside visual information. Evaluated on four complex real-world tasks involving credit card swiping, plug insertion, USB insertion, and bookshelf retrieval, ViSk significantly outperforms both vision-only and optical tactile sensing based policies. Further analysis reveals that combining tactile and visual modalities enhances policy performance and spatial generalization, achieving an average improvement of 27.5% across tasks. https://visuoskin.github.io/

==> sections/background.tex <==
\section{Background}
\label{sec:background}

\method{} builds on several technical ideas in B1 and B2:

\subsection{Imitaton Learning}



\subsection{Transformer Based Behavior Cloning Architecture}



\subsection{Learning from Tactile Data}

==> sections/results.tex <==

% \begin{table*}[t]
% \centering
% \caption{Policy Performance}
% \label{tab:performance}
% \begin{tabular}{cccc|ccccc}
% \hline
% \multicolumn{4}{c|}{\textbf{Sensor Modalities}}                                                                                                                                                                                              & \multicolumn{5}{c}{\textbf{Policy performance ($\cdot / 30$)}}             \\ \hline
% \textbf{\begin{tabular}[c]{@{}c@{}}3rd Person\\ Camera\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Wrist\\ Camera\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Robot\\ Proprioception\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Tactile\\ Sensing\end{tabular}} & \textbf{Plug-in-Socket} & \textbf{Card Swipe} & \textbf{USB Insertion} & \textbf{Book Retrieval} \\ \hline
%   \greencheck & \redcross   & \redcross   & \redcross   &   & 4 &   &                 \\
%   \greencheck & \redcross   & \greencheck & \redcross &   & 5 &   &                 \\
%   \greencheck & \greencheck & \redcross   & \redcross   & 3 & 2 & 2 &                    \\
%   \greencheck & \greencheck & \greencheck & \redcross & 1 & 3 & 3 &                    \\ \hdashline
% \rowcolor[HTML]{EFEFEF}
%   \greencheck & \redcross   & \redcross   & \greencheck & 5 & 12,9 &   &                    \\
% \rowcolor[HTML]{EFEFEF}
%   \greencheck & \redcross & \greencheck & \greencheck &  &  & &                    \\ 
% \rowcolor[HTML]{EFEFEF}
%   \greencheck & \greencheck & \redcross & \greencheck & 11,9 & 6 & 9,8 &                    \\ 
% \rowcolor[HTML]{EFEFEF}
%   \greencheck & \greencheck & \greencheck & \greencheck &  &  & &                    \\ 

%   \hline
% \end{tabular}
% \end{table*}


% \begin{table*}[t!]
% \caption{Success rates of \method{} and our baselines for evaluations run on the xArm with \revisit{AnySkin} tactile sensor.}
% \label{tab:success}
% \centering
% \begin{tabular}{lcccccc}
%                 & \multicolumn{1}{l}{\textsc{M1}} & \multicolumn{1}{l}{M2} & \multicolumn{1}{l}{M3} & \multicolumn{1}{l}{M4} & \multicolumn{1}{l}{M5} & \multicolumn{1}{l}{\method{}} \\ \hline
% Plug Insertion   & xx/30                      & xx/30         & xx/30        & xx/30                                       & xx/30                    & \textbf{20/30}            \\
% Card Swiping & xx/30                      & xx/30         & xx/30          & xx/30                                       & xx/30                    & \textbf{21/30}            \\
% USB Insertion  & xx/30                      & xx/30         & xx/30          & xx/30                                       & xx/30                    & \textbf{17/30}            \\
% Jar Closing & xx/30 & xx/30 & xx/30 & xx/30 & xx/30 & \textbf{xx/30} \\
% Book Retrieval & xx/30 & xx/30 & xx/30 & xx/30 & xx/30 & \textbf{xx/30} \\
% Easy Task & xx/30 & xx/30 & xx/30 & xx/30 & xx/30 & \textbf{xx/30} \\
% \hline
% Avg. Success Rate    & 0.xx                     & 0.xx     &   0.xx             & 0.xx                                     & 0.xx                    & \textbf{0.xx}         
% \end{tabular}
% \end{table*}



% \begin{table}[t]
% \centering
% \caption{Digit comparison}
% \label{tab:digit_comparison}
% \begin{tabular}{cccccc}
%  Sensor & Plug Insertion & Card Swiping & USB Insertion & Book Retrieval \\ \midrule
% DIGIT                   &  & \\
% AnySkin                 &  &  \\ \hline
% \end{tabular}
% \end{table}

% \subsection{Baselines and Evaluation}
% We study the effectiveness of our method and compare against the baselines \revisit{(both in terms of modalities/setup as well as in terms of the method)} described below:

% In terms of methodology:

% \begin{italicenum}
%     \item MLP (BAKU)
%     \item BAKU + VQ-BeT Policy Head
%     \item BAKU + Diffusion Policy Head
%     \item Diffusion Transformer (DiT)
%     \item ACT - Tactile
% \end{italicenum}

% % One of these will be the base method - rest of them stay here

% % All modalities include 3 overhead cameras, 1 egocentric fisheye camera, proprioception, and tactile observations.

% Ablations with regards to camera and sensory modalities:
% \begin{italicenum}
%     \item Overhead Cameras Only
%     \item Overhead Cameras + Proprioception
%     \item Overhead Cameras + Egocentric Camera
%     \item Overhead Cameras + Proprioception + Egocentric Camera
%     \item Overhead Cameras + Proprioception + Tactile
%     \item Overhead Cameras + Egocentric Camera + Tactile Single Frame
%     \item Overhead Cameras + Egocentric Camera + Tactile History (S4/LSTM)
%     \item Overhead Cameras + Egocentric Camera + High-Frequency Tactile History (S4/LSTM)
%     \item Tactile Only
% \end{italicenum}

